Unsupervised Image Prior via Prompt Learning and CLIP Semantic Guidance for Low-Light Image Enhancement

Currently, low-light conditions present a significant challenge for machine cognition. In this paper, rather than optimizing models by assuming that human and machine cognition are correlated, we use zero-reference low-light enhancement to improve the performance of downstream task models. We propose to improve the zero-reference low-light enhancement method by leveraging the rich visual-linguistic CLIP prior without any need for paired or unpaired normal-light data, which is laborious and difficult to collect. We propose a simple but effective strategy to learn prompts that help guide the enhancement method and experimentally show that the prompts learned without any need for normal-light data improve image contrast, reduce over-enhancement, and reduce noise over-amplification. Next, we propose to reuse the CLIP model for semantic guidance via zero-shot open vocabulary classification to optimize low-light enhancement for task-based performance rather than human visual perception. We conduct extensive experimental results showing that the proposed method leads to consistent improvements across various datasets regarding task-based performance and compare our method against state-of-the-art methods, showing favorable results across various low-light datasets.

==> Figures/Table_bp.tex <==
\begin{table*}[]
\centering
\small
\begin{tabular}{|cccc|ccccccc|}
\hline
Zero-ref. & Open vocab. & CLIP PSNR & Image & NOD & ExLPose BBox & LOD & ExDark & ExDark & DarkFace &  \\
baseline & classifier & classifier & TV Loss & mAP@.5:.95 & mAP@.5:.95 & mAP@.5:.95 & mAP@.5 & Classification & mAP@.5 &  \\ \hline
 &  &  &  & 42.1\% & 12.9\% & 37.8\% & 40.3\% & 22.8\% & 33.3\% &  \\
\checkmark &  &  &  & 40.4\% & 25.6\% & 38.6\% & 33.3\% & 40.9\% & 33.8\% &  \\
\checkmark &  &  & \checkmark & 42.5\% & 27.1\% & 44.7\% & 37.1\% & 47.0\% & 40.3\% &  \\
\checkmark & \checkmark &  &  & 41.1\% & 26.0\% & 42.5\% & 34.5\% & 41.2\% & 28.6\% &  \\
\checkmark & \checkmark &  & \checkmark & 42.6\% & 27.1\% & 46.4\% & 37.6\% & 47.0\% & 35.6\% &  \\
\checkmark &  & \checkmark &  & 42.4\% & 25.3\% & 47.1\% & 38.0\% & 42.7\% & 35.5\% &  \\
\checkmark &  & \checkmark & \checkmark & 43.4\% & 23.6\% & 46.6\% & 40.2\% & 40.5\% & 39.1\% &  \\
\checkmark & \checkmark & \checkmark &  & 43.2\% & 25.3\% & 47.4\% & 39.7\% & 43.6\% & 38.0\% &  \\
\checkmark & \checkmark & \checkmark & \checkmark & 43.5\% & 24.0\% & 44.6\% & 40.2\% & 36.0\% & 34.4\% &  \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table*}
